Approximate Policy Iteration Schemes: A Comparison

We consider the infinite-horizon discounted optimal control problem formalized by Markov Decision Processes. We focus on several approximate variations of the Policy Iteration algorithm: Approximate Policy Iteration, Conservative Policy Iteration (CPI), a natural adaptation of the Policy Search by Dynamic Programming algorithm to the infinite-horizon case (PSDP$_\infty$), and the recently proposed Non-Stationary Policy iteration (NSPI(m)). For all algorithms, we describe performance bounds, and make a comparison by paying a particular attention to the concentrability constants involved, the number of iterations and the memory required. Our analysis highlights the following points: 1) The performance guarantee of CPI can be arbitrarily better than that of API/API($\alpha$), but this comes at the cost of a relative---exponential in $\frac{1}{\epsilon}$---increase of the number of iterations. 2) PSDP$_\infty$ enjoys the best of both worlds: its performance guarantee is similar to that of CPI, but within a number of iterations similar to that of API. 3) Contrary to API that requires a constant memory, the memory needed by CPI and PSDP$_\infty$ is proportional to their number of iterations, which may be problematic when the discount factor $\gamma$ is close to 1 or the approximation error $\epsilon$ is close to $0$; we show that the NSPI(m) algorithm allows to make an overall trade-off between memory and performance. Simulations with these schemes confirm our analysis.

==> experiments.tex <==
\stretch
\section{Experiments}
\stretch

\labelsec{experiments}



\def\taille{0.95}

\newcommand{\showcurve}[3]{
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=\taille\textwidth]{#1.pdf}
\end{center}
\caption{#2 \label{#3}}
\end{figure}
}

\newcommand{\showcurveb}[6]{
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=\taille\textwidth]{#1.pdf}
\end{center}
\begin{center}
\includegraphics[width=\taille\textwidth]{#3.pdf}
\end{center}
\caption{#5 Top: #2. Bottom: #4.\label{#6}}
\end{figure}
}

\newcommand{\showcurvec}[8]{
\begin{figure}[ht!]
\begin{center}
\includegraphics[width=\taille\textwidth]{#1.pdf}
\end{center}
\begin{center}
\includegraphics[width=\taille\textwidth]{#3.pdf}
\end{center}
\begin{center}
\includegraphics[width=\taille\textwidth]{#5.pdf}
\end{center}
\caption{#7 Top: #2. Middle: #4. Bottom #6.\label{#8}}
\end{figure}
}


\showcurve{All}{Statistics for all instances}{expall}

%\showcurve{Hardest}{Statistics for one of the hardest instances}{exphard}

\showcurvec{S50}{$n_S=50$}{S100}{$n_S=100$}{S200}{$n_S=200$}{Statistics conditioned on the number of states.}{exps}

\showcurvec{A2}{$n_A=2$}{A5}{$n_A=5$}{A10}{$n_a=10$}{Statistics conditioned on the number of actions.}{expa}

\showcurvec{B1}{$b=1$ (deterministic)}{B2}{$b=2$}{B10}{$b=10$}{Statistics conditioned on the branching factor.}{expb}





In this section, we present some experiments in order to illustrate
the different algorithms discussed in the paper and to get some
insight on their empirical behaviour.  
We considered the standard API as a baseline.
CPI as it is described in
\refalgo{cpi} can be very slow (in one sample experiment on a 100
state problem, it made very slow progress and took several millions of
iterations before it stopped) and we did not evaluate it
further. Instead, we considered two variations: CPI+ that is identical
to CPI except that it chooses the step $\alpha$ at each iteration by
doing a line-search towards the policy output by the
classifier\footnote{We implemented a crude line-search mechanism, that
looks on the set $2^i \alpha$ where $\alpha$ is the minimal step
estimated by CPI to ensure improvement.}, and CPI($\alpha$) with
$\alpha=0.1$, that makes ``relatively but not too small'' steps at
each iteration. To assess the utility for CPI to use the distribution
$d_{\nu,\pi}$ for the approximate greedy step, we also considered
API($\alpha$) with $\alpha=0.1$, the variation of API described
in \refalgo{apialpha} that makes small steps, and that only differs
from CPI($\alpha$) by the fact that the approximate greedy step uses
the distribution $\nu$.  In addition to these algorithms, we
considered \PSDP{ }and \NSPI{ }for the values $m \in \{5,10,30\}$.
We begin by
describing the domain and the approximation considered.

\paragraph{Domain and Approximations}

In order to assess their quality, we consider finite problems where
the exact value function can be computed. More precisely, we consider
Garnet problems first introduced by \citet{Archibald:95}, which are a
class of randomly constructed finite MDPs. They do not correspond to
any specific application, but are totally abstract while remaining
representative of the kind of MDP that might be encountered in
practice. In our experiments, a Garnet is
parameterized by 4 parameters and is written $G(n_S, n_A, b, p)$:
$n_S$ is the number of states, $n_A$ is the number of actions, $b$ is
a branching factor specifying how many possible next states are
possible for each state-action pair ($b$ states are chosen uniformly
at random and transition probabilities are set by sampling uniform
random $b-1$ cut points between 0 and 1) and $p$ is the number of
features (for linear function approximation). The reward is
state-dependent: for a given randomly generated Garnet problem, the
reward for each state is uniformly sampled between 0 and 1. Features
are chosen randomly: $\Phi$ is a $n_S\times p$ feature matrix of which
each component is randomly and uniformly sampled between 0 and 1. The
discount factor $\gamma$ is set to $0.99$ in all experiments.

All the algorithms we have discussed in the paper need to repeatedly
compute $\greedy_\epsilon(\rho,v)$ for some distribution $\rho=\nu$ or
$\rho=d_{\pi,\nu}$. In other words, they must be able to make calls to
an approximate greedy operator applied to the value $v$ of some policy
for some distribution $\rho$. To implement this operator, we compute a
noisy estimate of the value $v$ with a uniform white noise $u(\iota)$
of amplitude $\iota$, then projects this estimate onto the space
spanned by $\Phi$ with respect to the $\rho$-quadratic norm
(projection that we write $\Pi_{\Phi,\rho}$), and then applies the
(exact) greedy operator on this projected estimate. In a nutshell, one
call to the approximate greedy operator $\greedy_\epsilon(\rho,v)$
amounts to compute $\greedy
\Pi_{\Phi,\rho}(v+u(\iota))$.


\paragraph{Simulations}

We have run series of experiments, in which we callibrated the
perturbations (noise, approximations) so that the algorithm are
significantly perturbed but no too much (we do not want their behavior
to become too erratic). After trial and error, we ended up considering
the following setting. We used Garnet problems $G(n_S, n_A, b, p)$
with the number of states $n_S \in \{50,100,200\}$, the number of actions
$n_A \in \{2, 5, 10\}$, the branching factor $b \in \{ 1,2,10 \}
\}$ ($b=1$ corresponds to deterministic problems), the number of
features to approximate the value $p=\frac{n_S}{10}$, and the noise
level $\iota=0.1$ ($10\%$).



For each of these $3^3=27$ parameter instances, we generated 30
i.i.d. Garnet MDPs $(M_i)_{1 \le i \le 30}$.  For each such MDP $M_i$,
we ran API, API(0.1), CPI+, CPI(0.1), \NSPI{ }for $m \in \{5,10,30\}$
and \PSDP{ }$30$ times. For each run $j$ and algorithm, we compute for
all iterations $k \in (1,100) $ the realization of the performance,
i.e. the loss $L_{j,k}=\mu(\v*-v_{\pi_k})$ with respect to the optimal
policy.  Figures \ref{expall} to \ref{expb} display statistics about
these random variables.  For each algorithm, we display a learning
curve with confidence regions.  The MDPs $(M_i)_{1 \le i \le 30}$ are
i.i.d. with the same distribution as $M_1$. Conditioned on some MDP
$M_i$ and some algorithm, the error measures at all iteration $k$ are
i.i.d. with the same distribution as $L_{1,k}$. The central line of
the learning curves gives the empirical estimate of the overall
average error $(\E[L_{1,k}])_k$. The three grey regions (from dark to
light grey) are estimates of respectively the variability (across
MDPs) of the average error $(\Std[\E[L_{1,k}|M_1]])_k$, the average
(across MDPs) of the standard deviation of the error
$(\E[\Std[L_{1,k}|M_1]])_k$, and the variability (across MDPs) of the
standard deviation of the error $(\Std[\Std[L_{1,k}|M_1]])_k$.  For
ease of comparison, all curves are displayed with the same $x$ and $y$
range. Figure~\ref{expall} shows the statistics overall for the
$3^3=27$ parameter instances. Figure~\ref{exps}, \ref{expa} and
\ref{expb} display statistics that are respectively conditioned on the
values of $n_S$, $n_A$ and $b$, which gives some insight
on the influence of these parameters.

From these experiments and statistics, we can make the following general
observations:
\begin{enumerate}
\item The standard API scheme is much more variable than the other
algorithms and tends to provide the worst performance on average.
\item CPI+ and CPI($\alpha$) display about the same asymptotic performance
on average. If CPI($\alpha$) has slightly less variability, it is much
slower than CPI+, that always converges in very few iterations (most
of the time less than 10, and always less than 20).
\item API($\alpha$) (the naive conservative variation of API that is also
simpler than CPI($\alpha$)) is empirically close to CPI($\alpha$),
while being on average slightly worse.
\item CPI+, CPI($\alpha$) and \PSDP{ }have a similar average performance,
but the variability of \PSDP{ }is consistantly smaller. \PSDP{ }is the
algorithm that overall gives the best results.
\item \NSPI{ }does indeed provide a bridge between API and \PSDP. By increasing $m$, the behavior
gets closer to that of \PSDP. With $m=30$, \NSPI{ }is overall better
than API($\alpha$), CPI+, and CPI(0.1), and close to \PSDP.
\item The above relative observations are rather stable with respect to the
number of states $n_S$ (Figure~\ref{exps}) and actions $n_A$
(Figure~\ref{expa}). Interestingly, the differences between the
algorithm tend to vanish when the dynamics of the problem gets more
and more stochastic (Figure~\ref{expb}). This is conform to our
analysis based on concentrability coefficients: there are all finite
when the dynamics mixes a lot, and their relative difference will be the
biggest in deterministic instances.
\end{enumerate}


==> proofs.tex <==
\section{Proof of \refth{api} (API)}

\labelapp{proofapi}

Our proof is here even slightly more general than what is required: we provide the result for any reference policy $\pi$ (and not only for the optimal policy $\pi_*$).
Writing $e_{k+1}=\max_{\pi'}T_{\pi'} v_{\pi_k} - T_{\pi_{k+1}} v_{\pi_k}$, we can first see that:
\begin{align}
v_{\pi}-v_{\pi_{k+1}} &= T_\pi v_\pi - T_\pi v_{\pi_k} + T_\pi v_{\pi_k} - T_{\pi_{k+1}} v_{\pi_k} +  T_{\pi_{k+1}} v_{\pi_k} - T_{\pi_{k+1}} v_{\pi_{k+1}} \\
& \le \gamma P_{\pi} (v_\pi-v_{\pi_k}) + e_{k+1} + \gamma P_{\pi_{k+1}}(v_{\pi_k}-v_{\pi_{k+1}}). \label{dpi:eq0}
\end{align}
Using the fact that $v_{\pi_{k+1}}=(I-\gamma P_{\pi_{k+1}})^{-1}r$, one can notice that:
\begin{align}
v_{\pi_k}-v_{\pi_{k+1}} & = (I-\gamma P_{\pi_{k+1}})^{-1}(v_{\pi_k}-\gamma P_{\pi_{k+1}}v_{\pi_k} - r) \\
& = (I-\gamma P_{\pi_{k+1}})^{-1}(T_{\pi_k}v_{\pi_k}-T_{\pi_{k+1}}v_{\pi_k}) \\
& \le (I-\gamma P_{\pi_{k+1}})^{-1}e_{k+1},
\end{align}
where we eventually used the fact that $(I-\gamma P_{\pi_{k+1}})^{-1}$ is non-negative.
Putting this back in \refequ{dpi:eq0} we get:
\begin{align}
v_{\pi}-v_{\pi_{k+1}} & \le \gamma P_{\pi} (v_\pi-v_{\pi_k}) +  (I-\gamma P_{\pi_{k+1}})^{-1} e_{k+1}.
\end{align}
Using the fact that $P_\pi$ is non-negative,  we obtain by induction on $k$:
\begin{align}
v_{\pi}-v_{\pi_{k}} &\le \sum_{i=0}^{k-1} (\gamma P_{\pi})^i (I-\gamma P_{\pi_{k-i}})^{-1} e_{k-i}   + (\gamma P_\pi)^k (v_{\pi}-v_{\pi_{0}}).
\end{align}
Multiplying both sides by $\mu$ (and observing that $e_k \ge 0$) and using \refdef{conc0} and the fact that $\nu e_j \le \epsilon_j$, we obtain:
\begin{align}
\mu(v_{\pi}-v_{\pi_{k}}) & \le \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i (I-\gamma P_{\pi_{k-i}})^{-1} e_{k-i}  + \gamma^k \vmax \\
& \le  \sum_{i=0}^{k-1} \left( \sum_{j=0}^\infty \gamma^{i+j} c(i+j) \epsilon_{k-i} \right) + \gamma^k \vmax \\
& = \sum_{i=0}^{k-1} \sum_{j=i}^\infty \gamma^j c(j) \epsilon_{k-i}  +  \gamma^k \vmax \label{dpi:eq1}\\
& \le  \sum_{i=0}^{k-1} \sum_{j=i}^\infty \gamma^j c(j) \max_{1 \le l \le k} \epsilon_l + \gamma^k \vmax, 
\end{align}
which provides the first bound.
Starting back on \refequ{dpi:eq1}, we get
\begin{align}
\mu(v_{\pi}-v_{\pi_{k}}) & \le  \sum_{i=0}^{k-1} \sum_{j=i}^\infty \gamma^j c(j) \epsilon_{k-i}  +  \gamma^k \vmax \\
& \le  \sum_{i=0}^{k-1} \sum_{j=0}^\infty \gamma^j c(j) \epsilon_{k-i}  +  \gamma^k \vmax \\
& = \left(\sum_{j=0}^\infty \gamma^j c(j)\right) \sum_{i=1}^k \epsilon_i + \gamma^k \vmax,
\end{align}
which proves the second bound.



\section{Proof of \refth{cpi} (CPI)}

\labelapp{proofcpi}

We include a concise and self-contained proof that essentially follows the steps in \citep{Kakade2002}.
 
(i) We first show that the value $\eta_k = \nu v_{\pi_k}$ is increasing along the iterations. 
Consider some iteration $k$ of the algorithm. Using the facts that $T_{\pi_{k+1}}v_{\pi_k} = (1-\alpha_{k+1}) v_{\pi_k} + \alpha_{k+1} T_{\pi'_{k+1}}v_{\pi_k}$ and $P_{\pi_{k+1}}=(1-\alpha_{k+1})P_{\pi_k}+\alpha_{k+1} P_{\pi'_{k+1}}$, we can see that:
\begin{align}
\eta_{k+1}-\eta_k &= \nu (v_{\pi_{k+1}}-v_{\pi_k}) \\
&= \nu [(I-\gamma P_{\pi_{k+1}})^{-1}r - v_{\pi_k}] \\
& = \nu (I-\gamma P_{\pi_k})^{-1}(I-\gamma P_{\pi_k})(I-\gamma P_{\pi_{k+1}})^{-1} [ r - (I-\gamma P_{\pi_{k+1}})v_{\pi_k}] \\
& = \nu (I-\gamma P_{\pi_k})^{-1}(I-\gamma P_{\pi_{k+1}}+\gamma P_{\pi_{k+1}}-\gamma P_{\pi_k})(I-\gamma P_{\pi_{k+1}})^{-1} (T_{\pi_{k+1}} v_{\pi_k} - v_{\pi_k}) \\
& = \frac{1}{1-\gamma}d_{\pi_k,\nu}\left[I+\gamma \alpha_{k+1} (P_{\pi'_{k+1}}-P_{\pi_k})(I-\gamma P_{\pi_{k+1}})^{-1}\right]\alpha_{k+1} (T_{\pi'_{k+1}} v_{\pi_k} - v_{\pi_k}) \\
& = \alpha_{k+1} \frac{1}{1-\gamma} d_{\pi_k,\nu}(T_{\pi'_{k+1}} v_{\pi_k} - v_{\pi_k}) + \alpha_{k+1}^2 \frac{\gamma}{1-\gamma} d_{\pi_k,\nu}(P_{\pi'_{k+1}}-P_{\pi_k})(I-\gamma P_{\pi_{k+1}})^{-1}(T_{\pi'_{k+1}} v_{\pi_k} - v_{\pi_k}) \\
& \ge \alpha_{k+1} \frac{1}{1-\gamma}(\hat \A_{k+1}-\frac{\rho}{3}) - 2\alpha_{k+1}^2 \frac{\gamma}{(1-\gamma)^2}\vmax 
\end{align}
where we eventually used the fact that $T_{\pi'_{k+1}} v_{\pi_k} - v_{\pi_k} \in (-\vmax,\vmax)$. Now, it can be seen that the setting $\alpha_{k+1}=\frac{(1-\gamma)(\hat \A_{k+1}-\frac{\rho}{3})}{4 \gamma \vmax}$ of \refalgo{cpi} is the one that maximizes the above right hand side. With this setting we get:
\begin{align}
\eta_{k+1}-\eta_k & \ge \frac{(\hat \A_{k+1}-\frac{\rho}{3})^2}{8 \gamma \vmax} \\
& > \frac{\rho^2}{72 \gamma \vmax}
\end{align} 
since as long as the algorithm iterates, $\hat \A_{k+1} > \frac{2\rho}{3}$.\\
(ii) The second point is a very simple consequence of (i): since $\eta_k = \nu v_{\pi_k} \le \vmax$, the number of iterations of the algorithm cannot exceed $\frac{72 \gamma \vmax^2}{\rho^2}$. \\
(iii) We now prove the performance bound. Write $e=\max_{\pi'}T_{\pi'} v_{\pi_{k^*}}-v_{\pi_{k^*}}$. We have:
\begin{align}
v_{\pi^*} - v_{\pi_{k^*}} & = T_{{\pi^*}}v_{\pi^*} - T_{{\pi^*}}v_{\pi_{k^*}} + T_{{\pi^*}}v_{\pi_{k^*}} - v_{\pi_{k^*}} \\
& \le \gamma P_{\pi^*} (v_{\pi^*} - v_{\pi_{k^*}}) + e \\
& \le (I-\gamma P_{\pi^*})^{-1} e,
\end{align}
where we eventually used the fact that $(I-\gamma P_{\pi^*})^{-1}$ is non-negative.
Multiplying by $\mu$, using \refdef{conc2} and the fact that $d_{\pi_{k^*},\nu} \ge (1-\gamma)\nu$, we obtain
\begin{align}
\mu(v_{\pi^*} - v_{\pi_{k^*}}) & \le \frac{1}{1-\gamma}d_{{\pi^*},\mu} e \\
& \le  \frac{\Cpi}{1-\gamma}\nu e \\
& \le \frac{\Cpi}{(1-\gamma)^2}d_{\pi_{k^*},\nu} e \\
& = \frac{\Cpi}{(1-\gamma)^2}d_{\pi_{k^*},\nu} (\max_{\pi'}T_{\pi'} v_{\pi_{k^*}} - T_{\pi'_{k^*+1}}v_{\pi_{k^*}} + T_{\pi'_{k^*+1}}v_{\pi_{k^*}} - v_{\pi_{k^*}}) \\
& \le \frac{\Cpi}{(1-\gamma)^2}(\epsilon_{k^*} + A_{k+1}).
\end{align}
Note that it is crucial that $e = \max_{\pi'}T_{\pi'} v_{\pi_{k^*}}-T_{\pi_{k^*}}v_{\pi_{k^*}}$ be non-negative for the second and third inequalities to hold.
The result follows by observing that the advantage satisfies $\A_{k+1} \le \hat \A_{k+1} + \frac{\rho}{3} \le \rho$ since $\hat \A_{k+1} \le \frac{2\rho}{3}$ when the algorithms stops.



\section{Proof of \refth{cpi2} (CPI($\alpha$))}

\labelapp{proofcpi2}

Using the facts that $T_{\pi_{k+1}} v_{\pi_k} = (1-\alpha_{k+1})v_{\pi_k}+\alpha_{k+1} T_{\pi_{k+1}} v_{\pi_k}$ and the notation $e_{k+1}=\max_{\pi'}T_{\pi'} v_{\pi_k} - T_{\pi'_{k+1}} v_{\pi_k}$, we have:
\begin{align}
v_\pi - v_{\pi_{k+1}} &= v_\pi - T_{\pi_{k+1}} v_{\pi_k} + T_{\pi_{k+1}} v_{\pi_k} - T_{\pi_{k+1}} v_{\pi_{k+1}} \\
& = v_\pi - (1-\alpha_{k+1})v_{\pi_k} - \alpha_{k+1} T_{\pi'_{k+1}} v_{\pi_k} + \gamma P_{\pi_{k+1}} (v_{\pi_k}-v_{\pi_{k+1}}) \\
& = (1-\alpha_{k+1}) (v_\pi - v_{\pi_k}) + \alpha_{k+1} (T_\pi v_\pi -  T_\pi v_{\pi_k}) +  \alpha_{k+1} (T_\pi v_{\pi_k} -  T_{\pi'_{k+1}} v_{\pi_k}) + \gamma P_{\pi_{k+1}} (v_{\pi_k}-v_{\pi_{k+1}}) \\
& \le \left[ (1-\alpha_{k+1})I+\alpha_{k+1}\gamma P_\pi \right](v_\pi-v_{\pi_k}) + \alpha_{k+1} e_{k+1} + \gamma P_{\pi_{k+1}} (v_{\pi_k}-v_{\pi_{k+1}}). \label{cpi:eq0}
\end{align}
Using the fact that $v_{\pi_{k+1}}=(I-\gamma P_{\pi_{k+1}})^{-1}r$, and the fact that $(I-\gamma P_{\pi_{k+1}})^{-1}$ is non-negative, we can see that
\begin{align}
v_{\pi_k}-v_{\pi_{k+1}} & = (I-\gamma P_{\pi_{k+1}})^{-1} (v_{\pi_k}-\gamma P_{\pi_{k+1}}v_{\pi_k}-r) \\
& = (I-\gamma P_{\pi_{k+1}})^{-1} (T_{\pi_k} v_{\pi_k}-T_{\pi_{k+1}}v_{\pi_k}) \\
& \le (I-\gamma P_{\pi_{k+1}})^{-1} \alpha_{k+1} e_{k+1}.
\end{align}
Putting this back in \refequ{cpi:eq0}, we obtain:
\begin{align}
v_\pi - v_{\pi_{k+1}} \le \left[ (1-\alpha_{k+1})I+\alpha_{k+1}\gamma P_\pi \right](v_\pi-v_{\pi_k}) + \alpha_{k+1} (I-\gamma P_{\pi_{k+1}})^{-1} e_{k+1}.
\end{align}
Define the matrix $Q_k=\left[ (1-\alpha_{k})I+\alpha_{k}\gamma P_\pi \right]$, the set ${\cal N}_{i,k}=\{j; k-i+1 \le j \le k\}$ (this set contains exactly $i$ elements), the matrix $R_{i,k}=\prod_{j \in {\cal N}_{i,k}} Q_j$, and the coefficients $\beta_k=1-\alpha_k(1-\gamma)$ and $\delta_k=\prod_{i=1}^k \beta_k$. By repeatedly using the fact that the matrices $Q_k$ are non-negative, we get by induction
\begin{align}
v_\pi - v_{\pi_{k}} \le \sum_{i=0}^{k-1} R_{i,k}  \alpha_{k-i} (I-\gamma P_{\pi_{k-i}})^{-1} e_{k-i} + \delta_k \vmax. \label{cpi:eq0}
\end{align}
Let ${\cal P}_j({\cal N}_{i,k})$ the set of subsets of  ${\cal N}_{i,k}$ of size $j$. With this notation we have
\begin{align}
R_{i,k} = \sum_{j=0}^{i} \sum_{I \in {\cal P}_j({\cal N}_{i,k})} \zeta_{I,i,k} (\gamma P_\pi)^j
\end{align}
where for all subset $I$ of ${\cal N}_{i,k}$, we wrote 
\begin{align}
\zeta_{I,i,k}=\left(\prod_{n \in I} \alpha_n \right) \left(\prod_{n \in {\cal N}_{i,k} \backslash I}(1-\alpha_n)\right).
\end{align}
Therefore, by multiplying \refequ{cpi:eq0} by $\mu$, using \refdef{conc0}, and the facts that $\nu \le (1-\gamma)d_{\nu,\pi_{k+1}}$, we obtain:
\begin{align}
\mu(v_\pi - v_{\pi_{k}}) & \le \frac{1}{1-\gamma} \sum_{i=0}^{k-1} \sum_{j=0}^{i} \sum_{l=0}^{\infty} \sum_{I \in {\cal P}_j({\cal N}_{i,k})} \zeta_{I,i,k} \gamma^{j+l}c(j+l) \alpha_{k-i} \epsilon_{k-i} + \delta_k \vmax. \\
& = \frac{1}{1-\gamma}  \sum_{i=0}^{k-1} \sum_{j=0}^{i} \sum_{l=j}^{\infty} \sum_{I \in {\cal P}_j({\cal N}_{i,k})} \zeta_{I,i,k} \gamma^{l}c(l) \alpha_{k-i} \epsilon_{k-i} + \delta_k \vmax \\
& \le \frac{1}{1-\gamma} \sum_{i=0}^{k-1} \sum_{j=0}^{i} \sum_{l=0}^{\infty} \sum_{I \in {\cal P}_j({\cal N}_{i,k})} \zeta_{I,i,k} \gamma^{l}c(l) \alpha_{k-i} \epsilon_{k-i} + \delta_k \vmax \\
 &= \frac{1}{1-\gamma} \left( \sum_{l=0}^{\infty}\gamma^{l} c(l) \right) \sum_{i=0}^{k-1} \left( \sum_{j=0}^{i} \sum_{I \in {\cal P}_j({\cal N}_{i,k})} \zeta_{I,i,k} \right) \alpha_{k-i} \epsilon_{k-i} + \delta_k \vmax \\
& = \frac{1}{1-\gamma} \left( \sum_{l=0}^{\infty}\gamma^{l} c(l) \right) \sum_{i=0}^{k-1} \left( \prod_{j \in  {\cal N}_{i,k}} (1-\alpha_j+\alpha_j) \right) \alpha_{k-i} \epsilon_{k-i} + \delta_k \vmax \\
& = \frac{1}{1-\gamma}  \left( \sum_{l=0}^{\infty}\gamma^{l} c(l) \right) \left( \sum_{i=0}^{k-1} \alpha_{k-i} \epsilon_{k-i} \right)  + \delta_k \vmax.
\end{align}

Now, using the fact that for $x \in (0,1)$, $\log(1-x) \le -x$, we can observe that
\begin{align}
\log \delta_k &= \log \prod_{i=1}^k \beta_i 
 = \sum_{i=1}^k \log \beta_i 
 = \sum_{i=1}^k \log(1-\alpha_i(1-\gamma)) 
 \le -(1-\gamma)\sum_{i=1}^k \alpha_i.
\end{align}
As a consequence, we get $\delta_k \le e^{-(1-\gamma)\sum_{i=1}^k \alpha_i}$.



\section{Proof of \refth{psdp} (\PSDP)}

\labelapp{proofpsdp}

As for the proof of CPI, we prove a slightly more general result that is true for any policy $\pi$ and not only for $\pi_*$ (we will thus refer to the straight-forward extension of the coefficients $c_\pi(\cdots)$ in \refdef{conc1}).
We begin by the first relation. For all $k$, we have
\begin{align}
v_\pi - v_{\sigma_{k}} &
=~ T_{\pi} v_\pi - T_{\pi}v_{\sigma_{k-1}} + T_{\pi}v_{\sigma_{k-1}} - T_{\pi_k}v_{\sigma_{k-1}} \\
&
\le~ \gamma P_{\pi} (v_\pi-v_{\sigma_{k-1}}) + e_k \label{eq0}
\end{align}
where we defined $e_k=\max_{\pi'}T_{\pi'}v_{\sigma_{k-1}} - T_{\pi_k}v_{\sigma_{k-1}}$.
As $P_\pi$ is non negative, we deduce by induction:
\begin{align}
v_\pi - v_{\sigma_k} \le~ \sum_{i=0}^{k-1} (\gamma P_{\pi})^i e_{k-i} + \gamma^k \vmax. 
\end{align}
By multiplying both sides by $\mu$, using \refdef{conc1} and the fact that $\nu_j e_j \le \epsilon_j$, we get:
\begin{align}
\mu(v_\pi - v_{\sigma_k}) &
\le~ \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i e_{k-i} + \gamma^k \vmax \label{eq1} \\
& 
\le~ \sum_{i=0}^{k-1} \gamma^i c_\pi(i) \epsilon_{k-i} + \gamma^k \vmax \\
&
\le~ \left(\sum_{i=0}^{k-1} \gamma^i c_\pi(i)\right) \max_{1 \le i \le k}\epsilon_i + \gamma^k \vmax.
\end{align}
We now prove the second relation. Starting back in \refequ{eq1} and using \refdef{conc2} (in particular the fact that for all $i$, $\mu(\gamma P_{\pi})^i \le \frac{1}{1-\gamma}d_{\pi^*,\mu} \le \frac{\Cpi}{1-\gamma}\nu$) and the fact that $\nu e_j \le \epsilon_j$, we get:
\begin{align}
\mu(v_\pi - v_{\sigma_k}) &
\le \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i e_{k-i} + \gamma^k \vmax \\
&
\le \frac{\Cpi}{1-\gamma}\sum_{i=1}^{k}\epsilon_i + \gamma^k \vmax
\end{align}
and the result is obtained by using the fact that $v_{\sigma_k \dots} \ge v_{\sigma_k} - \gamma^k \vmax$.


\section{Proof of \refth{nspi} (\NSPI)}

\labelapp{proofnspi}

Since \NSPI{ }reduces to API when $m=1$, the proof we are going to describe is a generalization of that provided for API in \refapp{proofapi}.
The beginning of the proof follows the lines of that provided by \citet{Scherrer:2012}. Some details differ because we here assume that we have an approximate greedy operator while \citet{Scherrer:2012} assumed they regress approximately the value of the non-stationary policy at each iteration. Also, and as before, we state it in a slightly more general way: for any policy $\pi$ instead of just the optimal policy $\pi_*$.

It will be convenient to introduce the following compound discounted kernel:
\begin{align*}
\Gamma_{k,m}=(\gamma P_{\pi_k}) (\gamma P_{\pi_{k-1}}) \cdots (\gamma P_{\pi_{k-m+1}}).
\end{align*}
In particular, for any pair of values $v$ and $v'$, it can easily be seen that $T_{k,m}v-T_{k,m}v'=\Gamma_{k,m}(v-v')$.

Using the facts that $T_{k+1,m+1}v_{\pi_{k,m}}=T_{\pi_{k+1}} T_{k,m}v_{\pi_{k,m}}=T_{\pi_{k+1}}v_{\pi_{k,m}}$ and writing $e_{k+1}=\max_{\pi'}T_{\pi'}v_{\pi_{k,m}} - T_{\pi_{k+1}}v_{\pi_{k,m}}$,  we have for $k \ge 0$,
\begin{align}
v_\pi - v_{\pi_{k+1,m}}  =&~ T_{\pi}v_\pi - T_{k+1,m} v_{\pi_{k+1,m}} \notag\\
=&~ T_{\pi}v_\pi - T_{\pi}v_{\pi_{k,m}} + T_{\pi}v_{\pi_{k,m}} - T_{k+1,m+1}v_{\pi_{k,m}} + T_{k+1,m+1}v_{\pi_{k,m}} - T_{k+1,m} v_{\pi_{k+1,m}}   \notag\\
=&~ \gamma P_{\pi} (v_\pi -  v_{\pi_{k,m}}) + T_{\pi}v_{\pi_{k,m}} - T_{\pi_{k+1}}v_{\pi_{k,m}} + \Gamma_{k+1,m}(T_{\pi_{k-m+1}} v_{\pi_{k,m}} - v_{\pi_{k+1,m}}) \notag\\
 \le&~ \gamma P_{\pi} (v_\pi -  v_{\pi_{k,m}}) + e_{k+1} +  \Gamma_{k+1,m}(T_{\pi_{k-m+1}} v_{\pi_{k,m}} - v_{\pi_{k+1,m}}). \label{nspi:eq1}
\end{align}
%%%
Consider the non-stationary policy
$$
\pi'_{k,m} ~=~ \pi_{k-m+1}\  \pi_{k}\  \dots\  \pi_{k+2-m}\  \pi_{k-m+1}\  \pi_{k}\  \dots\  \pi_{k-m+2} \dots
$$
that is essentially a 1-step right rotation of the policy $\pi_k,m$.
Since $\pi'_{k,m}$ takes the first action with respect to $\pi_{k-m+1}$ and then runs $\pi_{k,m}$, we have $v_{\pi'_{k,m}}=T_{\pi_{k-m+1}} v_{\pi_{k,m}}$.
As a consequence, Equation~\eqref{nspi:eq1} can be rewritten as follows:
\begin{align}
v_\pi - v_{\pi_{k+1,m}} & \le \gamma P_{\pi} (v_\pi -  v_{\pi_{k,m}}) + e_{k+1} + \Gamma_{k+1,m} (v_{\pi'_{k,m}}-v_{\pi_{k+1,m}}). \label{nspi:eq2}
\end{align}
Observe now that we have:
\begin{align*}
v_{\pi'_{k,m}}-v_{\pi_{k+1,m}} &= T_{\pi_{k-m+1}} v_{\pi_{k,m}} - v_{\pi_{k+1,m}} \\
& \le T_{\pi_{k+1}} v_{\pi_{k,m}} + e_{k+1} - v_{\pi_{k+1,m}} \\
& = T_{\pi_{k+1}} T_{k,m} v_{\pi_{k,m}} - T_{k+1,m} v_{\pi_{k+1,m}} +  e_{k+1}\\
& = T_{k+1,m} T_{\pi_{k-m+1}} v_{\pi_{k,m}} - T_{k+1,m} v_{\pi_{k+1,m}} + e_{k+1}\\
& = \Gamma_{k+1,m}(T_{\pi_{k-m+1}} v_{\pi_{k,m}} - v_{\pi_{k+1,m}}) + e_{k+1}\\
&= \Gamma_{k+1,m}(v_{\pi'_{k,m}} - v_{\pi_{k+1,m}}) + e_{k+1}
\end{align*}
from which we deduce that:
\begin{align*}
v_{\pi'_{k,m}} - v_{\pi_{k+1,m}} \le (I-\Gamma_{k+1,m})^{-1} e_{k+1}
\end{align*}
Putting this back in \refequ{nspi:eq2}, and using the fact that $P_\pi$ and $(I-\Gamma_{k+1,m})^{-1}$ are non-negative, we get:
\begin{align*}
v_\pi - v_{\pi_{k+1,m}} & \le \gamma P_{\pi} (v_\pi -  v_{\pi_{k,m}}) + e_{k+1} + \Gamma_{k+1,m} (I-\Gamma_{k+1,m})^{-1} e_{k+1} \\
& = \gamma P_{\pi} (v_\pi -  v_{\pi_{k,m}}) + (I-\Gamma_{k+1,m})^{-1} e_{k+1}.
\end{align*}
Using again the fact that $P_\pi$ is non-negative, we deduce by induction on $k$ that:
\begin{align}
v_{\pi}-v_{\pi_{k,m}} &\le \sum_{i=0}^{k-1} (\gamma P_{\pi})^i (I-\Gamma_{k-i,m})^{-1} e_{k-i}   + (\gamma P_\pi)^k (v_{\pi}-v_{\pi_{0,m}}).
\end{align}
To ease the arguments, we shall assume that $\epsilon_{-k}=0$ for all $k \ge 0$. Multiplying both sides by $\mu$ (and observing that $e_k \ge 0$) and using \refdef{conc0} and the fact that $\nu e_j \le \epsilon_j$, we obtain:
\begin{align}
\mu(v_{\pi}-v_{\pi_{k}}) & \le \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i(I-\Gamma_{k-i,m})^{-1} e_{k-i}  + \gamma^k \vmax \label{nspi:eq4}\\
& \le  \sum_{i=0}^{k-1} \left( \sum_{j=0}^\infty \gamma^{i+jm} c(i+jm) \epsilon_{k-i} \right) + \gamma^k \vmax  \label{nspi:eq3} \\
& \le  \sum_{i=0}^{k-1} \sum_{j=0}^\infty \gamma^{i+jm} c(i+jm) \max_{1 \le l \le k} \epsilon_l + \gamma^k \vmax, \label{nspi:eq5}
\end{align}
which provides the first bound.
Starting back on \refequ{nspi:eq3}, we get
\begin{align}
\mu(v_{\pi}-v_{\pi_{k}}) & = \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil}\sum_{h=0}^{m-1}  \sum_{j=0}^\infty  \gamma^{h+(l+j)m} c(h+(l+j)m) \epsilon_{k-h-lm}  +  \gamma^k \vmax\\ 
& \le \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil}\sum_{h=0}^{m-1}  \sum_{j=l}^\infty  \gamma^{h+jm} c(h+jm) \max_{k-(l+1)m+1 \le p \le k-lm} \epsilon_p +  \gamma^k \vmax\\ 
& \le \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil}\sum_{h=0}^{m-1}  \sum_{j=0}^\infty  \gamma^{h+jm} c(h+jm) \max_{k-(l+1)m+1 \le p \le k-lm} \epsilon_p +  \gamma^k \vmax\\ 
& = \left( \sum_{h=0}^{m-1}  \sum_{j=0}^\infty  \gamma^{h+jm} c(h+jm) \right)  \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil}\max_{l-(l+1)m+1 \le p \le k-lm} \epsilon_p +  \gamma^k \vmax \\
& = \left( \sum_{i=0}^{\infty}   \gamma^{i} c(i) \right) \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil} \max_{k-(l+1)m+1 \le p \le k-lm} \epsilon_p +  \gamma^k \vmax, \label{nspi:eq6}
\end{align}
which proves the second bound. Last but not least, starting back on \refequ{nspi:eq4}, and using the fact that $(I-\Gamma_{k-i,m})^{-1}=I+\Gamma_{k-i,m}(I-\Gamma_{k-i,m})^{-1}$ we see that:
\begin{align}
\mu(v_{\pi}-v_{\pi_{k}}) & \le \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i e_{k-i} + \sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i\Gamma_{k-i,m}(I-\Gamma_{k-i,m})^{-1} e_{k-i}  + \gamma^k \vmax. 
\end{align}
The first term of the r.h.s. can be bounded exactly as for \PSDP{ } in \refapp{proofpsdp}. For the second term, we have:
\begin{align}
\sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i\Gamma_{k-i,m}(I-\Gamma_{k-i,m})^{-1} e_{k-i} & \le \sum_{i=0}^{k-1} \sum_{j=1}^\infty \gamma^{i+jm} c(i+jm) \epsilon_{k-i} \\
& = \gamma^m \sum_{i=0}^{k-1} \sum_{j=0}^\infty \gamma^{i+jm} c(i+(j+1)m) \epsilon_{k-i},
\end{align}
and we follow the same lines as above (from \refequ{nspi:eq3} to Equations~\eqref{nspi:eq5} and~\eqref{nspi:eq6}) to conclude that:
\begin{align}
\sum_{i=0}^{k-1} \mu (\gamma P_{\pi})^i\Gamma_{k-i,m}(I-\Gamma_{k-i,m})^{-1} e_{k-i} & \le 
\left\{
\begin{array}{l}
\sum_{i=0}^{k-1} \sum_{j=0}^\infty \gamma^{i+jm} c(i+j(m+1)) \max_{1 \le l \le k} \epsilon_l  \\
\left( \sum_{i=0}^{\infty}   \gamma^{i} c(i+m) \right) \sum_{l=0}^{\left\lceil \frac{k-1}{m}\right\rceil} \max_{k-(l+1)m+1 \le p \le k-lm} \epsilon_p.
\end{array}
\right.
\end{align}


